An exact finite-state representation of viscoelastic memory for accelerated sea-level modeling: SLEvolve v1.0

Glacial Isostatic Adjustment (GIA) models solve the gravitationally self-consistent sea-level equation for the response of the solid Earth and the oceans to changing ice loads. As these models are increasingly embedded in coupled ice-sheet simulations, glacial-cycle calculations, and large ensembles, standard pseudo-spectral 1-D solvers face a steep computational barrier: they evaluate the viscoelastic response by explicitly re-summing every past load increment, scaling quadratically with time steps as $O(N^2)$. Here we show that this computational penalty is an artifact of algorithmic formulation rather than Earth physics. By exploiting the exponential form of the viscoelastic relaxation kernel, we reformulate the viscous response as an exact recursive update of a finite set of modal states, without re-summing the load history. This exact reformulation alone reduces the cost of a run to $O(N)$, yielding a 20.6-fold speed-up relative to a standard full-history 1-D GIA solver for a case study involving a 550-step Antarctic future sea-level projection. Implemented in our open-source solver SLEvolve v1.0, this formulation---combined with fewer, table-free and multithreaded spherical-harmonic transforms, improved file handling, and physics-inspired iteration starts---achieves an end-to-end speed-up of over three orders of magnitude (up to 4,000-fold) against the same 1-D GIA solver, reducing day-long simulations to under thirty seconds on a workstation. Beyond this solid-Earth application, SLEvolve illustrates how human-derived analytical reformulations can be combined with benchmark-harnessed AI-assisted engineering to modernize scientific software. In particular, Numerical regression tests and performance profiling guided the AI agents' implementation choices and helped reject ineffective optimizations.

==> copernicus_config.tex <==
\newif\ifprp             \DeclareOption{prp}     {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue                  \@bartrue \prptrue}
\newif\ifgtes            \DeclareOption{gtes}    {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue                  \@bartrue \gtestrue}
\newif\ifdwes            \DeclareOption{dwes}    {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@twostagejnltrue \@barfalse\dwestrue}
                         \DeclareOption{dwesd}   {\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@stage@finalfalse          \dwestrue}
\newif\ifproofreadingchanges    \DeclareOption{proofreadingchanges}{\proofreadingchangestrue\@noreftrue}
\newif\ifcopyediting     \DeclareOption{copyediting}{\copyeditingtrue\@noreftrue}
\newif\ifsmsps           \DeclareOption{smsps}   {                  \smspstrue}
\newif\ifls  \DeclareOption{ls}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@seclinetrue\@twostagejnltrue\lstrue}
            \DeclareOption{lsd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@stage@finalfalse\lstrue}
\newif\ifeo  \DeclareOption{eo}{\@sansseriffacetrue\@sansserifheadertrue\@firstbartrue\@twostagejnltrue\eotrue}
            \DeclareOption{eod}{\@sansseriffacetrue\@sansserifheadertrue\@firstbartrue\@stage@finalfalse\eotrue}
\newif\ifjecats  \DeclareOption{jecats}{\@sansseriffacetrue\@sansserifheadertrue\@twostagejnltrue\jecatstrue}
            \DeclareOption{jecatsd}{\@sansseriffacetrue\@sansserifheadertrue\@stage@finalfalse\jecatstrue}
\newif\ifpiodp  \DeclareOption{piodp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\piodptrue}
\newif\ifar  \DeclareOption{ar}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@twostagejnltrue\artrue}
            \DeclareOption{ard}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@stage@finalfalse\artrue}
\newif\ifsp  \DeclareOption{sp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@twostagejnltrue\sptrue}
            \DeclareOption{spd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@stage@finalfalse\sptrue}
\newif\ifegusphere  \DeclareOption{egusphere}{\@twostagejnltrue\eguspheretrue}
            \DeclareOption{egusphered}{\@stage@finalfalse\eguspheretrue}
\newif\ifsand  \DeclareOption{sand}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\sandtrue}
            \DeclareOption{sandd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\sandtrue}
\newif\ifpolf  \DeclareOption{polf}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\polftrue}
\newif\ifjbji  \DeclareOption{jbji}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\jbjitrue}
\newif\ifmr  \DeclareOption{mr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\mrtrue}
            \DeclareOption{mrd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\mrtrue}
\newif\ifejm  \DeclareOption{ejm}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\ejmtrue}
\newif\ifwcd  \DeclareOption{wcd}{\@twostagejnltrue\wcdtrue}
            \DeclareOption{wcdd}{\@stage@finalfalse\wcdtrue}
\newif\ifgchron  \DeclareOption{gchron}{\@sansseriffacetrue\@sansserifheadertrue\@twostagejnltrue\gchrontrue}
            \DeclareOption{gchrond}{\@sansseriffacetrue\@sansserifheadertrue\@stage@finalfalse\gchrontrue}
\newif\ifdeuquasp  \DeclareOption{deuquasp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@seclinetrue\deuquasptrue}
\newif\ifgc  \DeclareOption{gc}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\@twostagejnltrue\gctrue}
            \DeclareOption{gcd}{\@sansseriffacetrue\@sansserifheadertrue\@bartrue\@stage@finalfalse\gctrue}
\newif\ifegqsj  \DeclareOption{egqsj}{\@sansseriffacetrue\@sansserifheadertrue\@abstractindentedtrue\@bartrue\@seclinetrue\egqsjtrue}
\newif\ifjm  \DeclareOption{jm}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\jmtrue}
\newif\ifwes  \DeclareOption{wes}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\westrue}
            \DeclareOption{wesd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\westrue}
\newif\ifaab  \DeclareOption{aab}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\aabtrue}
\newif\ifpiahs  \DeclareOption{piahs}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\piahstrue}
\newif\ifascmo  \DeclareOption{ascmo}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@corrigendumtrue\@editorialnotetwoctrue\ascmotrue}
\newif\ifsoil  \DeclareOption{soil}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\soiltrue}
            \DeclareOption{soild}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\soiltrue}
\newif\ifangeocom  \DeclareOption{angeocom}{\@bartrue\@twostagejnltrue\angeocomtrue}
            \DeclareOption{angeocomd}{\@bartrue\@stage@finalfalse\angeocomtrue}
\newif\ifwe  \DeclareOption{we}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\wetrue}
\newif\ifsdpd  \DeclareOption{sdpd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdpdtrue}
\newif\ifsdwr  \DeclareOption{sdwr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdwrtrue}
\newif\ifsdtd  \DeclareOption{sdtd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdtdtrue}
\newif\ifsdpr  \DeclareOption{sdpr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdprtrue}
\newif\ifsdsr  \DeclareOption{sdsr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\sdsrtrue}
\newif\ifasr  \DeclareOption{asr}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\asrtrue}
\newif\ifms  \DeclareOption{ms}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@twostagejnltrue\mstrue}
            \DeclareOption{msd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@stage@finalfalse\mstrue}
\newif\ifjsss  \DeclareOption{jsss}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\jssstrue}
\newif\ifhgss  \DeclareOption{hgss}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\hgsstrue}
            \DeclareOption{hgssd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\hgsstrue}
\newif\ifgh  \DeclareOption{gh}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\ghtrue}
\newif\ifesurf  \DeclareOption{esurf}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\esurftrue}
            \DeclareOption{esurfd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\esurftrue}
\newif\ifessd  \DeclareOption{essd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@twostagejnltrue\essdtrue}
            \DeclareOption{essdd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@stage@finalfalse\essdtrue}
\newif\iftc  \DeclareOption{tc}{\@twostagejnltrue\tctrue}
            \DeclareOption{tcd}{\@stage@finalfalse\tctrue}
\newif\ifse  \DeclareOption{se}{\@bartrue\@twostagejnltrue\setrue}
            \DeclareOption{sed}{\@bartrue\@stage@finalfalse\setrue}
\newif\ifos  \DeclareOption{os}{\@twostagejnltrue\ostrue}
            \DeclareOption{osd}{\@stage@finalfalse\ostrue}
\newif\ifnpg  \DeclareOption{npg}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@editorialnotedtrue\@twostagejnltrue\npgtrue}
            \DeclareOption{npgd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@stage@finalfalse\npgtrue}
\newif\ifnhess  \DeclareOption{nhess}{\@editorialnotedtrue\@twostagejnltrue\nhesstrue}
            \DeclareOption{nhessd}{\@stage@finalfalse\nhesstrue}
\newif\ifhess  \DeclareOption{hess}{\@twostagejnltrue\hesstrue}
            \DeclareOption{hessd}{\@stage@finalfalse\hesstrue}
\newif\ifgmd  \DeclareOption{gmd}{\@firstbartrue\@twostagejnltrue\gmdtrue}
            \DeclareOption{gmdd}{\@firstbartrue\@stage@finalfalse\gmdtrue}
\newif\ifgi  \DeclareOption{gi}{\@corrigendumtrue\@editorialnotetwoctrue\@editorialnotedtrue\@twostagejnltrue\gitrue}
            \DeclareOption{gid}{\@stage@finalfalse\gitrue}
\newif\ifesd  \DeclareOption{esd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@twostagejnltrue\esdtrue}
            \DeclareOption{esdd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@bartrue\@stage@finalfalse\esdtrue}
\newif\ifcp  \DeclareOption{cp}{\@sansseriffacetrue\@sansserifheadertrue\@twostagejnltrue\cptrue}
            \DeclareOption{cpd}{\@sansseriffacetrue\@sansserifheadertrue\@stage@finalfalse\cptrue}
\newif\ifastra  \DeclareOption{astra}{\astratrue}
\newif\ifars  \DeclareOption{ars}{\arstrue}
\newif\ifangeo  \DeclareOption{angeo}{\@twostagejnltrue\angeotrue}
            \DeclareOption{angeod}{\@stage@finalfalse\angeotrue}
\newif\ifamt  \DeclareOption{amt}{\@twostagejnltrue\amttrue}
            \DeclareOption{amtd}{\@stage@finalfalse\amttrue}
\newif\ifadgeo  \DeclareOption{adgeo}{\adgeotrue}
\newif\ifbg  \DeclareOption{bg}{\@firstbartrue\@twostagejnltrue\bgtrue}
            \DeclareOption{bgd}{\@firstbartrue\@stage@finalfalse\bgtrue}
\newif\ifacp  \DeclareOption{acp}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@twostagejnltrue\acptrue}
            \DeclareOption{acpd}{\@sansseriffacetrue\@sansserifheadertrue\@abstractcenteredtrue\@firstbartrue\@stage@finalfalse\acptrue}



\def\@addjournalconfig{%


\ifcopyediting% Definition of layout used for copy-editing track changes document
  \def\@journalurl{}
  \def\@sentence{\textcolor[rgb]{1,0.58,0.25}{%
    Copy-Editing track changes document -- Do not use for proof-reading}}
  \let\@journalnameabbreviation\@sentence
  \if@sansserifface
    \definecolor{textcol}{rgb}{0,0,0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{gray}{0.8}
    \definecolor{rulecol}{gray}{0.8}
  \fi
\fi
\ifproofreadingchanges% Definition of layout used for proofreading changes document
  \def\@journalurl{}
  \def\@sentence{\textcolor[rgb]{1,0.58,0.25}{%
    Track changes document -- Do not use for proofreading}}
  \let\@journalnameabbreviation\@sentence
  \if@sansserifface
    \definecolor{textcol}{rgb}{0,0,0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{gray}{0.8}
    \definecolor{rulecol}{gray}{0.8}
  \fi
\fi

\ifacp%classical
  \def\@journalname{Atmospheric Chemistry and Physics}
  \def\@journalnameabbreviation{Atmos. Chem. Phys.}
  \def\@journalnameshort{ACP}
  \def\@journalnameshortlower{acp}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.atmos-chem-phys.net}
    \def\@journallogo{\includegraphics{ACP_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.447,0.737}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.447,0.737}
  \else
    \def\@journalurl{www.atmos-chem-phys-discuss.net}
    \def\@journallogo{\includegraphics{ACPD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Atmospheric Chemistry\\ and Physics (ACP). Please refer to the corresponding final paper in ACP if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.58,0.91}
      \definecolor{buttonbackground}{rgb}{0.0,0.58,0.91}
      \definecolor{paneltext}{rgb}{0.0,0.58,0.91}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifbg%classical
  \def\@journalname{Biogeosciences}
  \def\@journalnameabbreviation{Biogeosciences}
  \def\@journalnameshort{BG}
  \def\@journalnameshortlower{bg}
  \def\@journalstartyear{2004}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.biogeosciences.net}
    \def\@journallogo{\includegraphics{BG_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.0,0.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.612,0.698,0.145}
  \else
    \def\@journalurl{www.biogeosciences-discuss.net}
    \def\@journallogo{\includegraphics{BGD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Biogeosciences (BG).\\ Please refer to the corresponding final paper in BG if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.612,0.698,0.145}
      \definecolor{buttonbackground}{rgb}{0.612,0.698,0.145}
      \definecolor{paneltext}{rgb}{0.612,0.698,0.145}
      \definecolor{buttontext}{rgb}{0.612,0.0,0.055}
    \fi
  \fi
\fi
\ifadgeo%classical
  \def\@journalname{Advances in Geosciences}
  \def\@journalnameabbreviation{Adv. Geosci.}
  \def\@journalnameshort{ADGEO}
  \def\@journalnameshortlower{adgeo}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \def\@journalurl{www.adv-geosci.net}
  \def\@journallogo{\includegraphics{ADGEO_Logo.pdf}}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifamt%classical
  \def\@journalname{Atmospheric Measurement Techniques}
  \def\@journalnameabbreviation{Atmos. Meas. Tech.}
  \def\@journalnameshort{AMT}
  \def\@journalnameshortlower{amt}
  \def\@journalstartyear{2008}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.atmos-meas-tech.net}
    \def\@journallogo{\includegraphics{AMT_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.atmos-meas-tech-discuss.net}
    \def\@journallogo{\includegraphics{AMTD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Atmospheric Measurement\\ Techniques (AMT). Please refer to the corresponding final paper in AMT if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.259,0.475}
      \definecolor{buttonbackground}{rgb}{0.0,0.259,0.475}
      \definecolor{paneltext}{rgb}{0.0,0.259,0.475}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifangeo%classical
  \def\@journalname{Annales Geophysicae}
  \def\@journalnameabbreviation{Ann. Geophys.}
  \def\@journalnameshort{ANGEO}
  \def\@journalnameshortlower{angeo}
  \def\@journalstartyear{1983}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ann-geophys.net}
    \def\@journallogo{\includegraphics{ANGEO_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifars%classical
  \def\@journalname{Advances in Radio Sciences}
  \def\@journalnameabbreviation{Adv. Radio Sci.}
  \def\@journalnameshort{ARS}
  \def\@journalnameshortlower{ars}
  \def\@journalstartyear{2003}
  \def\@sentence{Published by Copernicus Publications on behalf of the URSI Landesausschuss in der Bundesrepublik Deutschland e.V.}
  \def\@journalurl{www.adv-radio-sci.net}
  \def\@journallogo{\includegraphics{ARS_Logo.pdf}}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifastra%classical
  \def\@journalname{Astrophysics and Space Sciences Transactions}
  \def\@journalnameabbreviation{Astrophys. Space Sci. Trans.}
  \def\@journalnameshort{ASTRA}
  \def\@journalnameshortlower{astra}
  \def\@journalstartyear{2004}
  \def\@sentence{Published by Copernicus Publications on behalf of the Arbeitsgemeinschaft Extraterrestrische Forschung e.V.}
  \def\@journalurl{www.astrophys-space-sci-trans.net}
  \def\@journallogo{}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifcp%classical
  \def\@journalname{Climate of the Past}
  \def\@journalnameabbreviation{Clim. Past}
  \def\@journalnameshort{CP}
  \def\@journalnameshortlower{cp}
  \def\@journalstartyear{2005}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.clim-past.net}
    \def\@journallogo{\includegraphics{CP_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.357,0.039,0.475}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.clim-past-discuss.net}
    \def\@journallogo{\includegraphics{CPD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Climate of the Past (CP).\\ Please refer to the corresponding final paper in CP if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.357,0.039,0.475}
      \definecolor{buttonbackground}{rgb}{0.357,0.039,0.475}
      \definecolor{paneltext}{rgb}{0.357,0.039,0.475}
      \definecolor{buttontext}{rgb}{1.0,0.796,0.02}
    \fi
  \fi
\fi
\ifesd%classical
  \def\@journalname{Earth System Dynamics}
  \def\@journalnameabbreviation{Earth Syst. Dynam.}
  \def\@journalnameshort{ESD}
  \def\@journalnameshortlower{esd}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.earth-syst-dynam.net}
    \def\@journallogo{\includegraphics{ESD_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.224,0.455}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.224,0.455}
  \else
    \def\@journalurl{www.earth-syst-dynam-discuss.net}
    \def\@journallogo{\includegraphics{ESDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth System\\ Dynamics (ESD). Please refer to the corresponding final paper in ESD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.224,0.455}
      \definecolor{buttonbackground}{rgb}{0.0,0.224,0.455}
      \definecolor{paneltext}{rgb}{0.0,0.224,0.455}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifgi%classical
  \def\@journalname{Geoscientific Instrumentation, Methods and Data Systems}
  \def\@journalnameabbreviation{Geosci. Instrum. Method. Data Syst.}
  \def\@journalnameshort{GI}
  \def\@journalnameshortlower{gi}
  \def\@journalstartyear{2012}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-instrum-method-data-syst.net}
    \def\@journallogo{\includegraphics{GI_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.geosci-instrum-method-data-syst-discuss.net}
    \def\@journallogo{\includegraphics{GID_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geoscientific Instrumentation,\\ Methods and Data Systems (GI). Please refer to the corresponding final paper in GI if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.012,0.306,0.635}
      \definecolor{buttonbackground}{rgb}{0.635,0.635,0.635}
      \definecolor{paneltext}{rgb}{0.012,0.306,0.635}
      \definecolor{buttontext}{rgb}{0.012,0.306,0.635}
    \fi
  \fi
\fi
\ifgmd%classical
  \def\@journalname{Geoscientific Model Development}
  \def\@journalnameabbreviation{Geosci. Model Dev.}
  \def\@journalnameshort{GMD}
  \def\@journalnameshortlower{gmd}
  \def\@journalstartyear{2008}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-model-dev.net}
    \def\@journallogo{\includegraphics{GMD_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.0,0.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.973,0.584,0.055}
  \else
    \def\@journalurl{www.geosci-model-dev-discuss.net}
    \def\@journallogo{\includegraphics{GMDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geoscientific Model\\ Development (GMD). Please refer to the corresponding final paper in GMD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.973,0.584,0.055}
      \definecolor{buttonbackground}{rgb}{0.973,0.584,0.055}
      \definecolor{paneltext}{rgb}{0.973,0.584,0.055}
      \definecolor{buttontext}{rgb}{0.769,0.086,0.11}
    \fi
  \fi
\fi
\ifhess%classical
  \def\@journalname{Hydrology and Earth System Sciences}
  \def\@journalnameabbreviation{Hydrol. Earth Syst. Sci.}
  \def\@journalnameshort{HESS}
  \def\@journalnameshortlower{hess}
  \def\@journalstartyear{1997}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.hydrol-earth-syst-sci.net}
    \def\@journallogo{\includegraphics{HESS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.hydrol-earth-syst-sci-discuss.net}
    \def\@journallogo{\includegraphics{HESSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Hydrology and Earth System\\ Sciences (HESS). Please refer to the corresponding final paper in HESS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.38,0.643,0.161}
      \definecolor{buttonbackground}{rgb}{0.38,0.643,0.161}
      \definecolor{paneltext}{rgb}{0.38,0.643,0.161}
      \definecolor{buttontext}{rgb}{0.122,0.153,0.498}
    \fi
  \fi
\fi
\ifnhess%classical
  \def\@journalname{Natural Hazards and Earth System Sciences}
  \def\@journalnameabbreviation{Nat. Hazards Earth Syst. Sci.}
  \def\@journalnameshort{NHESS}
  \def\@journalnameshortlower{nhess}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.nat-hazards-earth-syst-sci.net}
    \def\@journallogo{\includegraphics{NHESS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.nat-hazards-earth-syst-sci-discuss.net}
    \def\@journallogo{\includegraphics{NHESSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Natural Hazards and Earth\\ System Sciences (NHESS). Please refer to the corresponding final paper in NHESS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.263,0.416,0.702}
      \definecolor{buttonbackground}{rgb}{0.69,0.639,0.576}
      \definecolor{paneltext}{rgb}{0.263,0.416,0.702}
      \definecolor{buttontext}{rgb}{0.263,0.416,0.702}
    \fi
  \fi
\fi
\ifnpg%classical
  \def\@journalname{Nonlinear Processes in Geophysics}
  \def\@journalnameabbreviation{Nonlin. Processes Geophys.}
  \def\@journalnameshort{NPG}
  \def\@journalnameshortlower{npg}
  \def\@journalstartyear{1994}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union \& the American Geophysical Union.}
  \if@stage@final
    \def\@journalurl{www.nonlin-processes-geophys.net}
    \def\@journallogo{\includegraphics{NPG_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.102,0.278,0.6}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.102,0.278,0.6}
  \else
    \def\@journalurl{www.nonlin-processes-geophys-discuss.net}
    \def\@journallogo{\includegraphics{NPGD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Nonlinear Processes\\ in Geophysics (NPG). Please refer to the corresponding final paper in NPG if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.102,0.278,0.6}
      \definecolor{buttonbackground}{rgb}{0.996,0.749,0.004}
      \definecolor{paneltext}{rgb}{0.102,0.278,0.6}
      \definecolor{buttontext}{rgb}{0.102,0.278,0.6}
    \fi
  \fi
\fi
\ifos%classical
  \def\@journalname{Ocean Science}
  \def\@journalnameabbreviation{Ocean Sci.}
  \def\@journalnameshort{OS}
  \def\@journalnameshortlower{os}
  \def\@journalstartyear{2005}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ocean-sci.net}
    \def\@journallogo{\includegraphics{OS_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.ocean-sci-discuss.net}
    \def\@journallogo{\includegraphics{OSD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Ocean Science (OS).\\ Please refer to the corresponding final paper in OS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.039,0.282,0.494}
      \definecolor{buttonbackground}{rgb}{0.039,0.282,0.494}
      \definecolor{paneltext}{rgb}{0.039,0.282,0.494}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifse%classical
  \def\@journalname{Solid Earth}
  \def\@journalnameabbreviation{Solid Earth}
  \def\@journalnameshort{SE}
  \def\@journalnameshortlower{se}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.solid-earth.net}
    \def\@journallogo{\includegraphics{SE_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.solid-earth-discuss.net}
    \def\@journallogo{\includegraphics{SED_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Solid Earth (SE).\\ Please refer to the corresponding final paper in SE if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.482,0.349,0.259}
      \definecolor{buttonbackground}{rgb}{0.482,0.349,0.259}
      \definecolor{paneltext}{rgb}{0.482,0.349,0.259}
      \definecolor{buttontext}{rgb}{0.98,0.922,0.835}
    \fi
  \fi
\fi
\iftc%classical
  \def\@journalname{The Cryosphere}
  \def\@journalnameabbreviation{The Cryosphere}
  \def\@journalnameshort{TC}
  \def\@journalnameshortlower{tc}
  \def\@journalstartyear{2007}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.the-cryosphere.net}
    \def\@journallogo{\includegraphics{TC_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.the-cryosphere-discuss.net}
    \def\@journallogo{\includegraphics{TCD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal The Cryosphere (TC).\\ Please refer to the corresponding final paper in TC if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.341,0.596,0.824}
      \definecolor{buttonbackground}{rgb}{0.341,0.596,0.824}
      \definecolor{paneltext}{rgb}{0.341,0.596,0.824}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifessd%classical
  \def\@journalname{Earth System Science Data}
  \def\@journalnameabbreviation{Earth Syst. Sci. Data}
  \def\@journalnameshort{ESSD}
  \def\@journalnameshortlower{essd}
  \def\@journalstartyear{2009}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{www.earth-syst-sci-data.net}
    \def\@journallogo{\includegraphics{ESSD_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.102,0.4,0.573}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.earth-syst-sci-data-discuss.net}
    \def\@journallogo{\includegraphics{ESSDD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth System Science\\ Data (ESSD). Please refer to the corresponding final paper in ESSD if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.102,0.4,0.573}
      \definecolor{buttonbackground}{rgb}{0.102,0.4,0.573}
      \definecolor{paneltext}{rgb}{0.102,0.4,0.573}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifesurf%classical
  \def\@journalname{Earth Surface Dynamics}
  \def\@journalnameabbreviation{Earth Surf. Dynam.}
  \def\@journalnameshort{ESURF}
  \def\@journalnameshortlower{esurf}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.earth-surf-dynam.net}
    \def\@journallogo{\includegraphics{ESURF_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.541,0.549,0.557}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.earth-surf-dynam-discuss.net}
    \def\@journallogo{\includegraphics{ESURFD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Earth Surface Dynamics (ESurfD).\\ Please refer to the corresponding final paper in ESurf if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.0,0.0}
      \definecolor{buttonbackground}{rgb}{0.541,0.549,0.557}
      \definecolor{paneltext}{rgb}{0.0,0.0,0.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifgh%classical
  \def\@journalname{Geographica Helvetica}
  \def\@journalnameabbreviation{Geogr. Helv.}
  \def\@journalnameshort{GH}
  \def\@journalnameshortlower{gh}
  \def\@journalstartyear{1946}
  \def\@sentence{\small Published by Copernicus Publications for the Geographisch-Ethnographische Gesellschaft Z\"urich \& Association Suisse de G\'eographie.}
  \def\@journalurl{www.geogr-helv.net}
  \def\@journallogo{\includegraphics{GH_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.569,0.58,0.588}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.569,0.58,0.588}
\fi
\ifhgss%classical
  \def\@journalname{History of Geo- and Space Sciences}
  \def\@journalnameabbreviation{Hist. Geo Space Sci.}
  \def\@journalnameshort{HGSS}
  \def\@journalnameshortlower{hgss}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{www.hist-geo-space-sci.net}
    \def\@journallogo{\includegraphics{HGSS_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.443,0.706}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.443,0.706}
  \else
    \def\@journalurl{https://hgss.copernicus.org/preprints/preprints.html}
    \def\@journallogo{\includegraphics{HGSSD_Logo.pdf}}
    \def\@sentenceDiscussion{This preprint is/has been under review for the journal History of Geo- and Space Sciences (HGSS). Please refer to the corresponding final paper in HGSS if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifjsss%classical
  \def\@journalname{Journal of Sensors and Sensor Systems}
  \def\@journalnameabbreviation{J. Sens. Sens. Syst.}
  \def\@journalnameshort{JSSS}
  \def\@journalnameshortlower{jsss}
  \def\@journalstartyear{2012}
  \def\@sentence{Published by Copernicus Publications on behalf of the AMA Association for Sensor Technology.}
  \def\@journalurl{www.j-sens-sens-syst.net}
  \def\@journallogo{\includegraphics{JSSS_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.051,0.298,0.561}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.051,0.298,0.561}
\fi
\ifms%classical
  \def\@journalname{Mechanical Sciences}
  \def\@journalnameabbreviation{Mech. Sci.}
  \def\@journalnameshort{MS}
  \def\@journalnameshortlower{ms}
  \def\@journalstartyear{2010}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{www.mech-sci.net}
    \def\@journallogo{\includegraphics{MS_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.145,0.22,0.325}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{0.0,0.0,0.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{\includegraphics{MSD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifasr%classical
  \def\@journalname{Advances in Science and Research}
  \def\@journalnameabbreviation{Adv. Sci. Res.}
  \def\@journalnameshort{ASR}
  \def\@journalnameshortlower{asr}
  \def\@journalstartyear{2007}
  \def\@sentence{Published by Copernicus Publications.}
  \def\@journalurl{www.adv-sci-res.net}
  \def\@journallogo{\includegraphics{ASR_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.004,0.302,0.545}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.004,0.302,0.545}
\fi
\ifsdsr%classical
  \def\@journalname{Scientific Drilling - Science Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.075,0.239,0.553}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.075,0.239,0.553}
\fi
\ifsdpr%classical
  \def\@journalname{Scientific Drilling - Progress Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.906,0.651,0.278}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.906,0.651,0.278}
\fi
\ifsdtd%classical
  \def\@journalname{Scientific Drilling - Technical Developments}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.722,0.094,0.141}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{0.722,0.094,0.141}
\fi
\ifsdwr%classical
  \def\@journalname{Scientific Drilling - Workshop Reports}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.486,0.298,0.216}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.486,0.298,0.216}
\fi
\ifsdpd%classical
  \def\@journalname{Scientific Drilling - Program Developments}
  \def\@journalnameabbreviation{Sci. Dril.}
  \def\@journalnameshort{SD}
  \def\@journalnameshortlower{sd}
  \def\@journalstartyear{2013}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP and the ICDP.}
  \def\@journalurl{www.sci-dril.net}
  \def\@journallogo{\includegraphics{SD_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.027,0.498,0.325}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.027,0.498,0.325}
\fi
\ifwe%classical
  \def\@journalname{Web Ecology}
  \def\@journalnameabbreviation{Web Ecol.}
  \def\@journalnameshort{WE}
  \def\@journalnameshortlower{we}
  \def\@journalstartyear{2001}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Ecological Federation (EEF).}
  \def\@journalurl{www.web-ecol.net}
  \def\@journallogo{\includegraphics{WE_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.2,0.6,0.2}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.2,0.6,0.2}
\fi
\ifangeocom%classical
  \def\@journalname{AnGeo Communicates}
  \def\@journalnameabbreviation{Ann. Geophys.}
  \def\@journalnameshort{ANGEOCOM}
  \def\@journalnameshortlower{angeo}
  \def\@journalstartyear{1983}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.ann-geophys.net}
    \def\@journallogo{\includegraphics{ANGEO_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{0.851,0.851,0.851}
    \definecolor{rulecol}{rgb}{0.0,0.0,0.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifsoil%classical
  \def\@journalname{SOIL}
  \def\@journalnameabbreviation{SOIL}
  \def\@journalnameshort{SOIL}
  \def\@journalnameshortlower{soil}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.soil-journal.net}
    \def\@journallogo{\includegraphics{SOIL_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.29,0.267,0.165}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.29,0.267,0.165}
  \else
    \def\@journalurl{www.soil-discuss.net}
    \def\@journallogo{\includegraphics{SOILD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal SOIL. Please refer to the\\ corresponding final paper in SOIL if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.29,0.267,0.165}
      \definecolor{buttonbackground}{rgb}{0.29,0.267,0.165}
      \definecolor{paneltext}{rgb}{0.29,0.267,0.165}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifascmo%classical
  \def\@journalname{Advances in Statistical Climatology, Meteorology and Oceanography}
  \def\@journalnameabbreviation{Adv. Stat. Clim. Meteorol. Oceanogr.}
  \def\@journalnameshort{ASCMO}
  \def\@journalnameshortlower{ascmo}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications.}
  \def\@journalurl{www.adv-stat-clim-meteorol-oceanogr.net}
  \def\@journallogo{\includegraphics{ASCMO_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.392,0.039,0.039}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.392,0.039,0.039}
\fi
\ifpiahs%classical
  \def\@journalname{Proceedings of the International Association of Hydrological Sciences}
  \def\@journalnameabbreviation{Proc. IAHS}
  \def\@journalnameshort{PIAHS}
  \def\@journalnameshortlower{piahs}
  \def\@journalstartyear{1924}
  \def\@sentence{Published by Copernicus Publications on behalf of the International Association of Hydrological Sciences.}
  \def\@journalurl{proc-iahs.net}
  \def\@journallogo{\includegraphics{PIAHS_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.553,0.035,0.035}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.553,0.035,0.035}
\fi
\ifaab%classical
  \def\@journalname{Archives Animal Breeding}
  \def\@journalnameabbreviation{Arch. Anim. Breed.}
  \def\@journalnameshort{AAB}
  \def\@journalnameshortlower{aab}
  \def\@journalstartyear{2015}
  \def\@sentence{Published by Copernicus Publications on behalf of the Research Institute for Farm Animal Biology (FBN).}
  \def\@journalurl{www.arch-anim-breed.net}
  \def\@journallogo{\includegraphics{AAB_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.6,0.0,0.0}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifwes%classical
  \def\@journalname{Wind Energy Science}
  \def\@journalnameabbreviation{Wind Energ. Sci.}
  \def\@journalnameshort{WES}
  \def\@journalnameshortlower{wes}
  \def\@journalstartyear{2016}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Academy of Wind Energy e.V.}
  \if@stage@final
    \def\@journalurl{www.wind-energ-sci.net}
    \def\@journallogo{\includegraphics{WES_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.075,0.263,0.565}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.075,0.263,0.565}
  \else
    \def\@journalurl{www.wind-energ-sci-discuss.net}
    \def\@journallogo{\includegraphics{WESD_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Wind Energy Science (WES).\\ Please refer to the corresponding final paper in WES if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.075,0.263,0.565}
      \definecolor{buttonbackground}{rgb}{0.075,0.263,0.565}
      \definecolor{paneltext}{rgb}{0.075,0.263,0.565}
      \definecolor{buttontext}{rgb}{0.584,0.761,0.239}
    \fi
  \fi
\fi
\ifjm%classical
  \def\@journalname{Journal of Micropalaeontology}
  \def\@journalnameabbreviation{J. Micropalaeontology}
  \def\@journalnameshort{JM}
  \def\@journalnameshortlower{jm}
  \def\@journalstartyear{1982}
  \def\@sentence{Published by Copernicus Publications on behalf of The Micropalaeontological Society.}
  \def\@journalurl{www.j-micropalaeontol.net/}
  \def\@journallogo{\includegraphics{JM_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.047,0.306,0.427}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{0.047,0.306,0.427}
\fi
\ifegqsj%classical
  \def\@journalname{E&G Quaternary Science Journal}
  \def\@journalnameabbreviation{E\&G Quaternary Sci. J.}
  \def\@journalnameshort{EGQSJ}
  \def\@journalnameshortlower{egqsj}
  \def\@journalstartyear{1951}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Quart\"arvereinigung (DEUQUA) e.V.}
  \def\@journalurl{www.eg-quaternary-sci-j.net}
  \def\@journallogo{\includegraphics{EGQSJ_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.0,0.459,0.722}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifgc%classical
  \def\@journalname{Geoscience Communication}
  \def\@journalnameabbreviation{Geosci. Commun.}
  \def\@journalnameshort{GC}
  \def\@journalnameshortlower{gc}
  \def\@journalstartyear{2018}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geosci-commun.net}
    \def\@journallogo{\includegraphics{GC_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.067,0.494,1.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{0.067,0.494,1.0}
  \else
    \def\@journalurl{www.geosci-commun-discuss.net}
    \def\@journallogo{\includegraphics{GCD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifdeuquasp%classical
  \def\@journalname{DEUQUA Special Publications}
  \def\@journalnameabbreviation{DEUQUA Spec. Pub.}
  \def\@journalnameshort{DEUQUASP}
  \def\@journalnameshortlower{deuquasp}
  \def\@journalstartyear{2018}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Quart\"arvereinigung (DEUQUA) e.V.}
  \def\@journalurl{www.deuqua-spec-pub.net}
  \def\@journallogo{\includegraphics{DEUQUASP_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.529,0.533,0.541}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifgchron%classical
  \def\@journalname{Geochronology}
  \def\@journalnameabbreviation{Geochronology}
  \def\@journalnameshort{GCHRON}
  \def\@journalnameshortlower{gchron}
  \def\@journalstartyear{2019}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.geochronology.net}
    \def\@journallogo{\includegraphics{GCHRON_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.447,0.247,0.329}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.geochronology-discuss.net}
    \def\@journallogo{\includegraphics{GCHROND_Logo.pdf}}
    \def\@sentenceDiscussion{This discussion paper is/has been under review for the journal Geochronology (GChron).\\ Please refer to the corresponding final paper in GChron if available.}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifwcd%classical
  \def\@journalname{Weather and Climate Dynamics}
  \def\@journalnameabbreviation{Weather Clim. Dynam.}
  \def\@journalnameshort{WCD}
  \def\@journalnameshortlower{wcd}
  \def\@journalstartyear{2019}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.weather-clim-dynam.net}
    \def\@journallogo{\includegraphics{WCD_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.weather-clim-dynam-discuss.net}
    \def\@journallogo{\includegraphics{WCDD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifejm%classical
  \def\@journalname{European Journal of Mineralogy}
  \def\@journalnameabbreviation{Eur. J. Mineral.}
  \def\@journalnameshort{EJM}
  \def\@journalnameshortlower{ejm}
  \def\@journalstartyear{1989}
  \def\@sentence{Published by Copernicus Publications on behalf of the European mineralogical societies DMG, SEM, SIMP \& SFMC.}
  \def\@journalurl{www.eur-j-mineral.net}
  \def\@journallogo{\includegraphics{EJM_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.075,0.447,0.722}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifmr%classical
  \def\@journalname{Magnetic Resonance}
  \def\@journalnameabbreviation{Magn. Reson.}
  \def\@journalnameshort{MR}
  \def\@journalnameshortlower{mr}
  \def\@journalstartyear{2020}
  \def\@sentence{Published by Copernicus Publications on behalf of the Groupement AMPERE.}
  \if@stage@final
    \def\@journalurl{www.magn-reson.net}
    \def\@journallogo{\includegraphics{MR_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.627,0.098,0.086}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{\includegraphics{MRD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifjbji%classical
  \def\@journalname{Journal of Bone and Joint Infection}
  \def\@journalnameabbreviation{J. Bone Joint Infect.}
  \def\@journalnameshort{JBJI}
  \def\@journalnameshortlower{jbji}
  \def\@journalstartyear{2016}
  \def\@sentence{Published by Copernicus Publications on behalf of EBJIS and MSIS.}
  \def\@journalurl{https://jbji.copernicus.org/}
  \def\@journallogo{\includegraphics{JBJI_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.161,0.337,0.361}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.161,0.337,0.361}
\fi
\ifpolf%classical
  \def\@journalname{Polarforschung - Journal of the German Society for Polar Research}
  \def\@journalnameabbreviation{Polarforschung}
  \def\@journalnameshort{POLF}
  \def\@journalnameshortlower{polf}
  \def\@journalstartyear{1931}
  \def\@sentence{Published by Copernicus Publications on behalf of the Deutsche Gesellschaft für Polarforschung e.V.}
  \def\@journalurl{https://polf.copernicus.org}
  \def\@journallogo{\includegraphics{POLF_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.306,0.525,0.682}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
\fi
\ifsand%classical
  \def\@journalname{Safety of Nuclear Waste Disposal}
  \def\@journalnameabbreviation{Saf. Nucl. Waste Disposal}
  \def\@journalnameshort{SAND}
  \def\@journalnameshortlower{sand}
  \def\@journalstartyear{2021}
  \def\@sentence{Published by Copernicus Publications on behalf of the Federal Office for the Safety of Nuclear Waste Management (BASE).}
  \if@stage@final
    \def\@journalurl{www.sand.copernicus.org}
    \def\@journallogo{\includegraphics{SAND_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.0,0.0,0.0}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.0,0.0,0.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifegusphere%classical
  \def\@journalname{EGUsphere}
  \def\@journalnameabbreviation{EGUsphere}
  \def\@journalnameshort{EGUSPHERE}
  \def\@journalnameshortlower{egusphere}
  \def\@journalstartyear{2022}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{https://egusphere.copernicus.org}
    \def\@journallogo{\includegraphics{EGUSPHERE_Logo.pdf}}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{https://egusphere.copernicus.org}
    \def\@journallogo{\includegraphics{EGUSPHERE_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{0.0,0.0,0.0}
      \definecolor{buttonbackground}{rgb}{0.0,0.0,0.0}
      \definecolor{paneltext}{rgb}{0.0,0.0,0.0}
      \definecolor{buttontext}{rgb}{0.0,0.0,0.0}
    \fi
  \fi
\fi
\ifsp%classical
  \def\@journalname{State of the Planet}
  \def\@journalnameabbreviation{State Planet}
  \def\@journalnameshort{SP}
  \def\@journalnameshortlower{sp}
  \def\@journalstartyear{2023}
  \def\@sentence{Published by Copernicus Publications.}
  \if@stage@final
    \def\@journalurl{https://sp.copernicus.org/}
    \def\@journallogo{\includegraphics{SP_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.008,0.239,0.365}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.008,0.239,0.365}
  \else
    \def\@journalurl{}
    \def\@journallogo{\includegraphics{SPD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifar%classical
  \def\@journalname{Aerosol Research}
  \def\@journalnameabbreviation{Aerosol Res.}
  \def\@journalnameshort{AR}
  \def\@journalnameshortlower{ar}
  \def\@journalstartyear{2023}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Aerosol Assembly (EAA).}
  \if@stage@final
    \def\@journalurl{https://ar.copernicus.org/}
    \def\@journallogo{\includegraphics{AR_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.369,0.522,0.671}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{0.369,0.522,0.671}
  \else
    \def\@journalurl{}
    \def\@journallogo{\includegraphics{ARD_Logo.pdf}}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifpiodp%classical
  \def\@journalname{Proceedings of the International Ocean Drilling Programme}
  \def\@journalnameabbreviation{Proc. Int. Ocean Drill. Prog.}
  \def\@journalnameshort{PIODP}
  \def\@journalnameshortlower{piodp}
  \def\@journalstartyear{2025}
  \def\@sentence{Published by Copernicus Publications on behalf of the IODP³ Science Office, University of Plymouth.}
  \def\@journalurl{www.proceedings-IODP3.net}
  \def\@journallogo{\includegraphics{PIODP_Logo.pdf}}
  \definecolor{textcol}{rgb}{0.267,0.475,0.573}
  \definecolor{bgcol}{rgb}{1,1,1}
  \definecolor{barcol}{rgb}{1.0,1.0,1.0}
  \definecolor{rulecol}{rgb}{0.267,0.475,0.573}
\fi
\ifjecats%classical
  \def\@journalname{Journal of Environmentally Compatible Air Transport System}
  \def\@journalnameabbreviation{J. Env. Com. Air Transp. Sys.}
  \def\@journalnameshort{JECATS}
  \def\@journalnameshortlower{jecats}
  \def\@journalstartyear{2025}
  \def\@sentence{Published by Copernicus Publications on behalf of the ECATS International Association.}
  \if@stage@final
    \def\@journalurl{www.j-env-com-air-transp-sys.net}
    \def\@journallogo{\includegraphics{JECATS_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.569,0.576,0.188}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifeo%classical
  \def\@journalname{Earth Observation}
  \def\@journalnameabbreviation{Earth Obs.}
  \def\@journalnameshort{EO}
  \def\@journalnameshortlower{eo}
  \def\@journalstartyear{2026}
  \def\@sentence{Published by Copernicus Publications on behalf of the European Geosciences Union.}
  \if@stage@final
    \def\@journalurl{www.earth-observation.net}
    \def\@journallogo{\includegraphics{EO_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.416,0.29,0.588}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{barcol}{rgb}{1.0,1.0,1.0}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{www.earth-observation-discuss.net}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi
\ifls%classical
  \def\@journalname{Land Systems}
  \def\@journalnameabbreviation{Land Syst.}
  \def\@journalnameshort{LS}
  \def\@journalnameshortlower{ls}
  \def\@journalstartyear{2026}
  \def\@sentence{Published by Copernicus Publications on behalf of Land Systems association ASBL.}
  \if@stage@final
    \def\@journalurl{www.land-systems.net}
    \def\@journallogo{\includegraphics{LS_Logo.pdf}}
    \definecolor{textcol}{rgb}{0.333,0.529,0.255}
    \definecolor{bgcol}{rgb}{1,1,1}
    \definecolor{rulecol}{rgb}{1.0,1.0,1.0}
  \else
    \def\@journalurl{}
    \def\@journallogo{}
    \def\@sentenceDiscussion{}
    \if@cop@home
      \definecolor{journalname}{rgb}{1.0,1.0,1.0}
      \definecolor{buttonbackground}{rgb}{1.0,1.0,1.0}
      \definecolor{paneltext}{rgb}{1.0,1.0,1.0}
      \definecolor{buttontext}{rgb}{1.0,1.0,1.0}
    \fi
  \fi
\fi

}
